SoK: Software Debloating Landscape and Future Directions

Software debloating seeks to mitigate security risks and improve performance by eliminating unnecessary code. In recent years, a plethora of debloating tools have been developed, creating a dense and varied landscape. Several studies have delved into the literature, focusing on comparative analysis of these tools. To build upon these efforts, this paper presents a comprehensive systematization of knowledge (SoK) of the software debloating landscape. We conceptualize the software debloating workflow, which serves as the basis for developing a multilevel taxonomy. This framework classifies debloating tools according to their input/output artifacts, debloating strategies, and evaluation criteria. Lastly, we apply the taxonomy to pinpoint open problems in the field, which, together with the SoK, provide a foundational reference for researchers aiming to improve software security and efficiency through debloating.

==> background.tex <==
\section{Background and Related Work} \label{sec:background}

\subsection{Software Complexity}
% The core idea that this section should convey is that the complexity of software involves more dependencies.

%software development lifecycle
Modern software relies heavily on third-party libraries that are often
built to provide extensive functionality. \textcolor{blue}{To easily incorporate such libraries into programs, developers often rely on tools such as Maven, NPM, and PyPI. While this promotes code reuse and accelerates development, it also introduces complexity due to the integration of diverse third-party components, each with its own set of dependencies and potential vulnerabilities. Consequently, security risks increase as the attack surface expands, necessitating thorough vetting and updating of dependencies. Moreover, the inclusion of unnecessary library features can lead to code bloat, increasing the application's size and potentially degrading performance. In the next section, we discuss security from the perspective of attack surface management.}

\subsection{Attack Surface Management}
As software has expanded its functionality to serve more users, the size and complexity of libraries and applications have grown dramatically over time, resulting in software bloat.
As mentioned earlier, software applications accumulate new features over time, however, only a small amount of the accumulated features are used by users~\cite{holzmann2015code}. These unused features increase the attack surface. For example, code reuse attacks can rely on any part of code that exists in the address space of a vulnerable process—even code that is not used by the application. Address Space Layout Randomization (ASLR) was introduced as a means of preventing attackers from reusing exploit code effectively against multiple instantiations of a single vulnerable program~\cite{snow2013just}.

Software debloating is a technique that helps prune a program's attack surface by removing extraneous code. However, this requires a mechanism to infer this functionality to code mapping based on an informal description of the necessary functionality. Debloating also complements Control-Flow Integrity (CFI), which ensures that indirect control-flow transfers only go to legitimate targets, preventing unexpected malicious behaviors~\cite{ligatti2005control}. For example, while CFI allows a transfer from an indirect call $i$ to function $A$ if $A$ is legitimate, debloating will disable the transfer and remove $A$ if $A$'s functionality is not necessary. As such, debloating enforces a coarse-grained CFI by limiting control-flow to the remaining code and simplifying analysis due to a smaller code base, while CFI provides a foundation for implementing debloating. In the next section, we describe the typical software debloating workflow.

%SBOM 

%debloating
%Code debloating improves security along two dimensions: codereuse reduction and bug reduction. First, code debloating reduces the amount of available code, making it harder for an attacker to find gadgets for a code-reuse attack. Second, feature based code debloating approaches reduce attack surface by removing potentially reachable buggy functionality, making it harder for the attacker to find an exploitable bug.

\subsection{Software Debloating}
\label{sec:software_debloating}

Software bloat refers to unnecessary functionalities and their corresponding software dependencies and components~\cite{holzmann2015code}. %The debloating process consists of two primary steps: first, identifying these extraneous dependencies, and second, proceeding to eliminate them. 
% however, the debloating process can be extremely challenging, as most programs and libraries do not come with a formal description of their functionality. Consequently, . But these various debloating tools adopted a similar workflow. 
To identify such bloats and eliminate them, developers use existing tools to take in a \emph{bloated artifact}, such as an application, container, or firmware, and then produce an \emph{output artifact} based on a specific debloating strategy that the tool employs. After that, the quality of the output artifact is assessed using various evaluation criteria. Typically, \emph{debloating strategy} receives another optional input to indicate the required functionality that should be preserved in the output artifact. The next section discusses the details of this debloating workflow in the context of the reviewed literature and our proposed taxonomy.

==> comparison_table_orig.tex <==
% \begin{table*}[]
\begin{sidewaystable}
\centering
\caption{Systematization of software debloating tools from collected papers}
\scalebox{0.65}{
\begin{tabular}{|l|l|l|llll|llllll|llllll|}
\hline
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{4}{c|}{} & \multicolumn{6}{c|}{Strategy} & \multicolumn{6}{c|}{} \\ \cline{8-13}
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{4}{c|}{\multirow{-2}{*}{Removal Granularity}} & \multicolumn{3}{c|}{Analysis} & \multicolumn{3}{c|}{Functionality} & \multicolumn{6}{c|}{\multirow{-2}{*}{Evaluation Criteria}} \\ \cline{4-19} 
\multicolumn{1}{|c|}{\multirow{-3}{*}{Tool}} & \multicolumn{1}{c|}{\multirow{-3}{*}{Venue}} & \multicolumn{1}{c|}{\multirow{-3}{*}{\shortstack{In/Out\\ Artifacts}}} & \multicolumn{1}{c|}{File} & \multicolumn{1}{c|}{Library} & \multicolumn{1}{c|}{BB} & Stmt & \multicolumn{1}{c|}{Static} & \multicolumn{1}{c|}{Dynamic} & \multicolumn{1}{c|}{ML-Assisted} & \multicolumn{1}{c|}{Config.} & \multicolumn{1}{c|}{Test cases} & \multicolumn{1}{c|}{Annotation} & \multicolumn{1}{c|}{Performance} & \multicolumn{1}{c|}{Security} & \multicolumn{1}{c|}{Robustness} & \multicolumn{1}{c|}{Usability} & \multicolumn{1}{c|}{Integration} & \multicolumn{1}{c|}{Sustainability} \\ \hline
LMCAS~\cite{LMCAS} & EuroS\&P'22 & S2B & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \yes & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \yes & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no \\ \hline
CHISEL~\cite{CHISEL} & CCS'18 & S2S & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \yes & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \no & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no \\ \hline
OCCAM~\cite{OCCAM} & Commun. ACM'23 & S2B & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \yes & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no \\ \hline

RAZOR~\cite{RAZOR} & USENIX Sec'19 & B2B & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \no & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \no & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no \\ \hline

Nibbler~\cite{Nibbler} & ACSAC'19 & B2B & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \no & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no \\ \hline
DeepOCCAM~\cite{DeepOCCAM} & MLforSystems'19 & S2B & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \yes & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no \\ \hline
BlankIt~\cite{BlankIt} & PLDI'20 & B2B & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \yes & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no \\ \hline
BLADE~\cite{BLADE} & SecDev'23 & S2S & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \yes & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \no & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no \\ \hline
Mininode~\cite{Mininode} & RAID'20 & S2S & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \no & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \no \\ \hline
C-Reduce~\cite{C-Reduce} & PLDI'12 & S2S & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \yes & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \no & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \no \\ \hline
Perses~\cite{Perses} & ICSE'18 & S2S & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \yes & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \no & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no \\ \hline
DomGad~\cite{DomGad} & ASE'20 & S2S & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \yes & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \yes & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no \\ \hline

Trimmer~\cite{Trimmer} & TSE'22 & S2B & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \yes & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \yes & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no \\ \hline

CONFINE~\cite{CONFINE} & RAID'20 & C2P & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \no & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \no & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \no \\ \hline
SPEAKER~\cite{speaker} & DIMVA'17 & C2P & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \no & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \no & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \no \\ \hline
Cimplifier~\cite{Cimplifier} & FSE'17 & C2C & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \no & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \no & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no \\ \hline
Temporal Specal.~\cite{temporal} & USENIX Sec'20 & S2P & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \no \\ \hline
NA~\cite{Energy} & ISLPED '01 & S2S & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \yes & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \yes & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \yes \\ \hline

$\mu$Trimmer~\cite{mTrimmer} & ASPLOS'22 & B2B & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \no & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \no & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \no \\ \hline
XDebloat~\cite{XDebloat} & TSE'21 & B2B & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \yes & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \yes & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no \\ \hline
RedDroid~\cite{RedDroid} & ISSRE'18 & B2B & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \no & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \no \\ \hline

BINTRIMMER~\cite{BINTRIMMER} & LNSC'19 & B2B & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \no & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \yes & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no \\ \hline
Slimium~\cite{Slimium} & CCS'20 & S2B & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \yes & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \yes & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no \\ \hline
NA~\cite{cf_trimming} & CCS'19 & B2B & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \yes & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \yes & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \no \\ \hline
BinRec~\cite{BinRec} & FEAST'18 & B2B & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \yes & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \yes & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \no \\ \hline
C2C~\cite{C2C} & CCS'22 & S2P & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \no & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \yes & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no \\ \hline
NA~\cite{Configuration-Driven} & EuroSec'19 & S2B & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \yes & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \no \\ \hline
CARVE~\cite{CARVE} & FEAST'19 & S2S & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \yes & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \yes & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \no \\ \hline
Piece-Wise~\cite{Piece-Wise} & USENIX Sec'18 & S2B & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \yes & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no \\ \hline
Ancile~\cite{Ancile} & CODASPY '21 & S2B & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \yes & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no \\ \hline
Saffire~\cite{Saffire} & EuroS\&P'20 & S2B & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \yes & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no \\ \hline
JSLIM~\cite{JSLIM} & EISA 2021 & S2S & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \no & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \no \\ \hline
PRAT~\cite{PRAT} & TOSEM'21 & S2B & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \yes & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \no & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \no \\ \hline
LightBlue~\cite{LightBlue} & USENIX Sec'21 & S2B, B2B & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \yes & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \no \\ \hline
IRQDebloat~\cite{IRQDebloat} & S\&P'22 & B2B & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \yes & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \no \\ \hline
DECAF~\cite{DECAF} & ICSE-SEIP'20 & B2B & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \no & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \yes & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \no \\ \hline

JReduce~\cite{JReduce} & FSE'19 & B2B & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \no & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \no & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no \\ \hline
PacJam~\cite{PacJam} & ASIACCS '22 & S2S & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \yes & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \no & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no \\ \hline
DEPCLEAN & \shortstack{Empir SE'21} & D2D & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \no & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \no \\ \hline
JDBL~\cite{JDBL} & \shortstack{ACM Transactions \\SE and Meth.'23} & S2B & \multicolumn{1}{l|}{\yes } & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \yes & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \no \\ \hline
JShrink~\cite{JShrink} & FSE'20 & B2B & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \yes & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \yes & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \no \\ \hline

jred~\cite{jred} & COMPSAC'16 & B2B & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \no & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} & \no \\ \hline

Hacksaw~\cite{Hacksaw} & CCS'23	 & S2B & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} &	\multicolumn{1}{l|}{\no} &	\multicolumn{1}{l|}{\no} &	\multicolumn{1}{l|}{\yes} &	\multicolumn{1}{l|}{\yes} &	\multicolumn{1}{l|}{\no} &	\multicolumn{1}{l|}{\no} &	\multicolumn{1}{l|}{\no} &	\multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\no} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} &	\multicolumn{1}{l|}{\no} &	\no \\ \hline


Picup~\cite{Picup} & FSE'23	& S2B & \multicolumn{1}{l|}{\no} &	\multicolumn{1}{l|}{\yes} &	\multicolumn{1}{l|}{\no} &	\multicolumn{1}{l|}{\no} &	\multicolumn{1}{l|}{\yes} &	\multicolumn{1}{l|}{\yes} &	\multicolumn{1}{l|}{\yes} &	\multicolumn{1}{l|}{\yes} &	\multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} &	\multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\yes} & \multicolumn{1}{l|}{\no} &	\multicolumn{1}{l|}{\no} & \no \\ \hline

\end{tabular}
}
\label{table:summary}
\end{sidewaystable}
% \end{table*}
